Modelling Clock Synchronization in the Chess gMAC WSN Protocol

We present a detailled timed automata model of the clock synchronization algorithm that is currently being used in a wireless sensor network (WSN) that has been developed by the Dutch company Chess. Using the Uppaal model checker, we establish that in certain cases a static, fully synchronized network may eventually become unsynchronized if the current algorithm is used, even in a setting with infinitesimal clock drifts.

==> eptcsdata.tex <==
\providecommand{\event}{S. Andova et.al. (Eds.): Workshop on Quantitative Formal Methods:\\ Theory and Applications (QFM'09) }
\providecommand{\volume}{13}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{41}
\providecommand{\eid}{4}
\pdfoutput=1

